Dual Codebook VQ: Enhanced Image Reconstruction with Reduced Codebook Size

Vector Quantization (VQ) techniques face significant challenges in codebook utilization, limiting reconstruction fidelity in image modeling. We introduce a Dual Codebook mechanism that effectively addresses this limitation by partitioning the representation into complementary global and local components. The global codebook employs a lightweight transformer for concurrent updates of all code vectors, while the local codebook maintains precise feature representation through deterministic selection. This complementary approach is trained from scratch without requiring pre-trained knowledge. Experimental evaluation across multiple standard benchmark datasets demonstrates state-of-the-art reconstruction quality while using a compact codebook of size 512 - half the size of previous methods that require pre-training. Our approach achieves significant FID improvements across diverse image domains, particularly excelling in scene and face reconstruction tasks. These results establish Dual Codebook VQ as an efficient paradigm for high-fidelity image reconstruction with significantly reduced computational requirements.

==> sec/1_intro_v2_S2.tex <==
\section{Introduction}
\label{sec:intro}

Vector Quantization (VQ)~\cite{gray1984vector} has emerged as a powerful technique for mapping high-dimensional continuous data into discrete latent spaces using a finite set of learned code vectors. By replacing input features with their nearest codebook entries, VQ enforces a discrete bottleneck that enables efficient and compact representations. This approach has proven invaluable in unsupervised learning, particularly for image generation tasks, as demonstrated by Vector Quantized Variational Autoencoders (VQ-VAE) and subsequent extensions like VQ-GAN, which have significantly advanced generative modeling capabilities~\cite{esser2021taming, van2017neural, razavi2019generating}.

Despite these successes, a persistent challenge in VQ-based methods is \textit{codebook collapse}—a phenomenon where only a small subset of code vectors receives meaningful updates during training while the majority remain underutilized. This imbalance fundamentally limits representation capacity and reconstruction quality, as empirical evidence has shown that models utilizing a larger proportion of their codebook consistently achieve better image fidelity and lower FID scores. The degradation in image quality stemming from codebook collapse has prompted numerous studies focused on enhancing codebook update mechanisms and quantization strategies~\cite{takida2022sq, zhang2023regularized, zheng2023online, zhang2024codebook, zhu2024scaling}.

Existing approaches to address this limitation broadly fall into two categories: deterministic methods that select and update the single best-matching code vector per input, and stochastic methods that update multiple code vectors per iteration through various non-deterministic selection strategies. While deterministic approaches excel at capturing fine-grained local features, they often suffer from limited codebook utilization. Conversely, stochastic methods achieve better codebook distribution but may compromise precision in local feature representation. Recent state-of-the-art models such as VQCT~\cite{zhang2024codebook} have attempted to overcome these limitations by incorporating pre-trained knowledge from language models, achieving impressive results but at the cost of substantially increased codebook size (6207 vectors) and domain-specific dependencies.
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{Fig/fig1.pdf}
    \caption{Overview of Dual Codebook Implementation}
    \label{fig:overview-architecture}
\end{figure}
In this paper, we propose a novel Dual Codebook \footnote{Code available at: \href{https://github.com/aauthors131/dual-codebook-vqgan}{https://github.com/aauthors131/dual-codebook-vqgan}}
mechanism that combines the strengths of both deterministic and stochastic approaches without relying on pre-trained knowledge. Our key insight is that effective image representation requires capturing both global context and local details—requirements that are difficult to satisfy with a single codebook update strategy. The Dual Codebook approach partitions the codebook into two complementary components: a global codebook updated via a lightweight transformer that concurrently refines all code vectors to maximize utilization, and a local codebook updated through traditional deterministic selection to preserve fine-grained details.

Our experiments across ADE20K~\cite{zhou2017scene,zhou2019semantic}, CelebA-HQ~\cite{liu2015deep}, and MS-COCO~\cite{lin2014microsoft} datasets demonstrate that this complementary approach significantly outperforms existing methods on multiple metrics. Our method achieves FID scores of 17.03, 8.61, and 4.19 respectively—surpassing the current state-of-the-art while using a remarkably compact codebook of only 512 vectors, which is less than one-tenth the size of VQCT's 6207 vectors. Notably, our approach also shows substantial improvements in reconstruction fidelity through reduced L1 and L2 losses across all evaluated datasets.

Our main contributions can be summarized as follows:
\begin{itemize}
    \item We introduce a Dual Codebook mechanism that effectively captures both global and local features by integrating transformer-based stochastic updates with deterministic selection, achieving superior reconstruction quality without increasing total codebook size or computational overhead.
    
    \item We demonstrate that our approach eliminates the need for pre-trained knowledge or domain-specific information, making it entirely dataset-agnostic while still outperforming methods that rely on external priors.
    
    \item Our comprehensive experiments show that the Dual Codebook approach significantly improves codebook utilization, resulting in state-of-the-art performance across multiple datasets and metrics despite using a substantially smaller codebook (512 vectors) than current leading methods.
\end{itemize}

Figure~\ref{Fig/Fig1.pdf} provides an overview of our Dual Codebook architecture, illustrating how the complementary update mechanisms work together to optimize both feature representation and codebook utilization.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/experiment_2s.tex <==
\section{Experiments}
\label{sec:experiment}
\subsection{Experimental Details}
\subsubsection{Implementation} The Dual Codebook approach is implemented by modifying the vector quantization function and making slight adjustments to the loss function in PyTorch. Our implementation is based on the VQ-GAN architecture with these targeted modifications. The model is developed with PyTorch Lightning API. All
experiments were conducted on an NVIDIA DGX A100 with 8, 80 GB A100 GPUs.
\subsubsection{Dataset} We assess our method on four publicly available datasets: ADE20K \cite{zhou2017scene,zhou2019semantic}, CelebA-HQ \cite{liu2015deep}, MSCOCO \cite{lin2014microsoft}, and CUB-200 \cite{WahCUB_200_2011}. Consistent with the approach in \cite{zhang2024codebook} all images are resized to 256 × 256 for experimental evaluation and the latent size is 16×16.
\subsubsection{Evaluation Metrics} We compared our method with five recent VQ-based models VQ-VAE \cite{van2017neural}, VQ-GAN \cite{esser2021taming}, Gumbel-VQ \cite{baevski2019vq}, CVQ \cite{zheng2023online}, and VQCT \cite{zhang2024codebook} and evaluated them with image reconstruction performance. Four evalution metrics is used including Frechet Inception Score (FID) \cite{heusel2017gans}, $l1$ , $l2$, and PSNR (Peak Signal to noise Ratio) to show the quality of reconstructed images.
\subsection{Main Results}
\subsubsection{Quantitative Evaluation}
We showed the main result of our evaluation in Table \ref{tab:results} where we compare the performance of our reconstructed images against five baseline models under the same compression ratio (( 768\times ), \textit{i.e.}, ( 256 \times 256 \times 3 \rightarrow 16 \times 16 )). As shown in the table, our Dual Codebook method outperforms state-of-the-art approaches across most evaluation metrics. Notably, our model demonstrates a significant performance margin compared to VQCT, on ADE20K \cite{zhou2017scene,zhou2019semantic} (17.03 vs. 20.25) and MS-COCO \cite{lin2014microsoft} (4.19 vs
9.82) datasets, highlighting its effectiveness in VQ-based models.
Despite utilizing a codebook of size 512—substantially smaller than VQCT \cite{zhang2024codebook}, which employs a codebook of size 6207 (1949 adjectives and 4258 nouns)—our method still achieves a notable improvement in FID and loss values. It is important to emphasize that, unlike VQCT, which leverages a pre-trained codebook prior for optimization, our Dual Codebook model is trained from scratch, further demonstrating its robustness and adaptability.
We also evaluated our method on the CUB-200 dataset \cite{WahCUB_200_2011}, which contains images of 200 bird species and presents unique challenges due to the complex textures and gradient color patterns in birds' feathers. The results in Table \ref{tab:cub200} reveal an interesting pattern: while our Dual Codebook approach achieves better pixel-wise accuracy with lower $l1$ and $l2$ losses compared to baseline methods, it does not attain the best FID scores. This suggests that our method captures local details accurately but may struggle with certain perceptual aspects of bird images, particularly the subtle gradient transitions that are characteristic of natural bird plumage.
\subsubsection{Qualitative Evaluation}
The qualitative evaluation of our model is shown in Figure~\ref{fig:qualitative-result} where we compare the reconstruction result of our model with the VQ-GAN as our baseline model on two different dataset ADE20k and MS-COCO. Compared to the baseline VQ-GAN, our model achieves superior reconstruction quality, particularly in preserving textures
and producing sharper details across different domain. This comparison highlights the effectiveness of our Dual Codebook approach in generating high-fidelity reconstructed images. Additionally, Figure~\ref{fig:_qualitative-result-cel} presents a comprehensive set of reconstruction results on CelebA-HQ dataset using our Dual Codebook method. The figure showcases both the best-case and worst-case reconstructions, providing a detailed qualitative analysis of our model's performance.
\begin{figure}
\centering
\includegraphics[width=\linewidth]{Fig/fig2.pdf}
\caption{Comparison of reconstructed images from our Dual Codebook and VQ-GAN on two datasets. Two models are trained under the same settings and same compression ration (( 768\times ), \textit{i.e.}, ( 256 \times 256 \times 3 \rightarrow 16 \times 16 )) but different codebook size (codebook size for VQ-GAN is 1024 and for Dual Codebook is 512). Our proposed quantization method substantially enhances reconstruction quality especially in the improved texture detail in building facades and the sky background in balcony for ADE20k dataset. In the second row for Ms-COCO in addition to the more detailed man anatomy, it shows better reconstruction detail and color in man's helmet.(the red boxed highlighted the reconstruction details).}
\label{fig:qualitative-result}
\end{figure}





\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Fig/supp_fig_1_cel-editted.pdf}
\caption{Best and worst reconstruction result on CelebA-HQ (test split) with Dual Codebook quantizer respectively first and second row (Best and worst case selected based on PSNR value).}
\label{fig:_qualitative-result-cel}
\end{figure*}
\subsection{Ablation Experiments}
\subsubsection{Dual Codebook Partition}
Table \ref{tab:codebook configuration} presents an ablation study evaluating the effectiveness of our Dual Codebook design in enhancing image quality. Specifically, we investigate (1) the impact of introducing global and local codebooks at varying ratios, and (2) the effectiveness of incorporating a transformer into the global codebook.
The experiment compares five configurations: (i) the baseline (VQ-GAN \cite{esser2021taming}); and four Dual Codebook variants using different channel allocations and transformer settings: (ii) 128-channel global and local codebooks without a transformer; (iii) a 192-channel transformer-based global codebook with a 64-channel simple local codebook; (iv) a 64-channel transformer-based global codebook with a 192-channel simple local codebook; and (v) 128-channel transformer-based global and simple local codebooks.
For the ablation study, we chose MS-COCO \cite{lin2014microsoft} as the primary dataset due to its extensive size and complexity, making it the most suitable for scene image reconstruction. As shown in Table~\ref{tab:codebook configuration}, row (i) and (ii) suggested having Dual Codebook yields good performance on all parameters, even without using any non-deterministic updating method like transformer. On the other hand,comparing (ii) and (v) suggested that having transformer-based global codebook resulted in better performance across all metrics. Additionally, having a a large rather than small global codebook yields better results across all evaluation metrics, as shown in comparing (iii) and (v) to (iv).
This study suggested that implementing Dual Codebook with large transformer-based global codebook size significantly improve model's performance. Between the configurations (iv) and (v), (iv) had slightly better FID value, but (v) presented better losses and PSNR values. Hence, we decided to use configuration (v) to implement the Dual Codebook for all experiments.
% By comparing (i) and (ii), we observe that introducing a Dual Codebook—even without a non-deterministic updating method such as a transformer—has a positive impact on all evaluation metrics, particularly the FID score. Next, we investigate whether employing a transformer for updating affects performance. Experiments (iii) and (iv) confirm that incorporating a transformer with different channel configurations (192 and 64) enhances image quality. Finally, in (v), we equally allocate channels between the global and local codebooks. While (iv) and (v) yield almost similar FID scores, experiment (v) also achieves favorable loss and PSNR values. Based on these findings, we adopt the configuration in (v) for all subsequent experiments.
\begin{table}
\centering
\small
\caption{Evaluation results of ablation study on MS-COCO dataset with four different codebook configuration. In Global and Local columns we have T for transformer based codebook and S for simple codebook method. In different models we split the 256 channels for global and local as it mentioned in the table. The best results are highlighted in bold. See Supplimental Figure~\ref{fig:supp1-ultility} for detailed codebook utility.}
\label{tab:codebook configuration}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l  c ccccc}
\toprule
Models & Global & Local  & FID$\downarrow$ & PSNR$\uparrow$ & $L_1\downarrow$ & $L_2\downarrow$ \
\midrule
Copy(i) VQ-GAN~\cite{esser2021taming} & - & - & 14.45 & 20.21 & 0.1311 & 0.0475\\
(ii) Dual Codebook &  S - 128 & S - 128 & 4.91 & 19.58 & 0.0857 & 0.0131  \\
(iii) Dual Codebook & T - 192 & S - 64 & 4.67 & 19.26 & 0.0865 & 0.0139\\
(iv) Dual Codebook & T - 64 & S - 192   & \textbf{4.12} & 19.51 & 0.0853 & 0.0133 \\
(v) Dual Codebook & T - 128 & S - 128 & 4.19 & \textbf{20.72} & \textbf{0.0717} & \textbf{0.0103}\\
\bottomrule
\end{tabular}
}
\end{table}
\subsubsection{Codebook Size}
The codebook size is a critical factor in the performance of VQ-based models, as it directly affects the expressiveness of the latent space and the quality of image reconstruction. However, a larger codebook size also requires significant system memory and computational resources, making it crucial to strike a balance between performance and efficiency. As a result, researchers often aim to optimize model performance while minimizing codebook size to reduce memory overhead and improve computational feasibility. In Table \ref{tab:codebook size}, we evaluate the performance of our Dual Codebook framework under different codebook sizes 1024 and 512. Our results indicate that increasing the codebook size enhances the model's performance in FID score (3.24), demonstrating high-quality image reconstruction. However, even with a smaller codebook size of 512, our method still maintains strong performance, ensuring competitive image quality while significantly reducing memory usage. These findings highlight the effectiveness and adaptability of the Dual Codebook framework, as it leverages an optimized quantization strategy that remains robust across different codebook sizes. The ability to maintain competitive performance with a smaller codebook size underscores its efficiency and scalability, making it a practical choice for memory-constrained environments.
\begin{table}
\centering
\small
\caption{Evaluation results of ablation study on MS-COCO dataset with codebook size of 1024 and 512. The best results are highlighted in bold.}
\label{tab:codebook size}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l ccccc}
\toprule
Models & Codebook Size  & FID$\downarrow$ & PSNR$\uparrow$ & $L_1\downarrow$ & $L_2\downarrow$ \
\midrule
(i) Dual Codebook & 1024 & \textbf{3.24} & 20.48 & 0.0751 & 0.0108\
(ii) Dual Codebook & 512  & 4.19 & \textbf{20.72} & \textbf{0.0717} & \textbf{0.0103} \
% (iii) Dual Codebook &  256 & - & - & - & - \
Copy\bottomrule
\end{tabular}
}
\end{table}
% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{Fig/fig-3.pdf}
%     \caption{Visualization of codebook (first row) and illustration of codebook usage (second row) on MS-COCO dataset for VQ-GAN (blue) and our Dual Codebook method (red and blue). In this comparison, VQ-GAN was tested with codebook size of 1024, but our Dual Codebook was teste with 512 codebook size totally (the red graph related to global codebook usage and blue one is for local codebook usage for Dual codebook).}
%     \label{fig:utility}
% \end{figure*}
\subsubsection{Codebook Utilization}
We also examined the impact of our Dual Codebook method on codebook utilization using the MS-COCO dataset. As shown in Figure~\ref{fig:utility}, we compare our model against vanilla VQ-GAN \cite{esser2021taming} with deterministic quantization. The first row of this figure presents the codebook visualizations for both methods, revealing a significant difference in codebook updates between our approach and VQ-GAN. In this row, the blue grids represent intact and inactive code vectors, highlighting the codebook collapse issue in VQ-GAN.
The second row illustrates the codebook usage for both models. The left blue graph (containing 1024 code vectors) depicts VQ-GAN's codebook usage, further demonstrating the codebook collapse issue. In contrast, the red and blue graphs (each with 512 code vectors) correspond to the global and local codebooks in our proposed quantization method, respectively. This figure provides clear evidence of the Dual Codebook quantization method's effectiveness in enhancing codebook utilization and improving reconstructed image quality.
